Backpropagating through Structured Argmax using a SPIGOT

We introduce the structured projection of intermediate gradients optimization technique (SPIGOT), a new method for backpropagating through neural networks that include hard-decision structured predictions (e.g., parsing) in intermediate layers. SPIGOT requires no marginal inference, unlike structured attention networks (Kim et al., 2017) and some reinforcement learning-inspired solutions (Yogatama et al., 2017). Like so-called straight-through estimators (Hinton, 2012), SPIGOT defines gradient-like quantities associated with intermediate nondifferentiable operations, allowing backpropagation before and after them; SPIGOT's proxy aims to ensure that, after a parameter update, the intermediate structure will remain well-formed. We experiment on two structured NLP pipelines: syntactic-then-semantic dependency parsing, and semantic parsing followed by sentiment classification. We show that training with SPIGOT leads to a larger improvement on the downstream task than a modularly-trained pipeline, the straight-through estimator, and structured attention, reaching a new state of the art on semantic dependency parsing.

==> response <==
R1

- RL does not always requires marginal inference. We will clarify this.

R1 rightly points out that if marginal inference has been done (as in, say, structured attention), then one could inspect the most probable intermediate output. But our argument is that that since in SA *all* possible intermediate outputs affect the end-task prediction, the 1-best intermediate parse may not be the source of the error.

- Yes, this sentence is meant to describe Eqn 4c. The RHS can be seen as the (projected) gradient of L w.r.t. \hat{z}. And this update rule resembles Eqn 3 (with J=I) in that they both pass the gradients w.r.t. \hat{z} straight through to the gradients w.r.t. s. We will clarify this connection.

- Right, SPIGOT can be used even when using an approximate decoder (like beam search) during the forward pass. We should clarify that AD3, the inference method in NeurboParser, is approximate, so our second set of experiments provide justification for this claim.

- PSD is another semantic dependency formalism from the SemEval shared task, derived from the Prague Czech-English Dependency Treebank.
We will introduce and cite it in our revision.

We thank reviewer #1 for their other helpful advice, which we will take!


R2

Reply to weakness argument 2: We will include more discussion on the theoretical justifications of SPIGOT.


R3

Reply to weakness argument 1 and question 1: We note theoretical connections between a class of differentiable quadratic programs (reviewed at around line 245) and SPIGOT. At a very high level, by assuming an invertible Hessian of the objective, the Jacobian of the structured argmax (denoted as J) can be explicitly formed by solving a linear system involving the Hessian. 
One can show that, in such cases, J projects the gradients w.r.t. \hat{z} onto the relaxed feasible set.
However, many NLP problems have linear objectives, and thus such a method does not apply.
Yet, it is still the theoretical motivation for SPIGOT, where a key step is to solving a projection onto the feasible set.
We will include such discussion using the additional space.

Reply to question 2: \eta is not necessarily the same as the overall learning rate.
It functions more as a ratio of intermediate learning rate to end-task learning rate (although because of the projection the relationship is not exactly linear). We tuned it based on dev set performance, using 1.0 and 5/32 respectively for the two experiments. We will clarify this point.


Reply to question 3: Thanks for pointing out this interesting connection! Eq.4c resembles a perceptron update by viewing \hat{z} as the prediction, and \tilde{z} as the desired output. Considering that perceptron can be extended to SVM's hinge loss, it would be interesting to investigate whether SPIGOT has an analogous margin-based extension.


==> reviews <==

Review #1
Appropriateness:	Appropriate
Adhere to ACL 2018 Guidelines:	Yes
Adhere to ACL Author Guidelines:	Yes
Handling of Data / Resources:	Yes
Handling of Human Participants:	N/A
Summary and Contributions

Summary: Proposes an alternative to the "straight through" estimator for calculating gradients for non-differentiable operators such as argmax. Evaluates on a couple of tasks set up as pipelines, with an argmax component as part of the pipeline. The tasks are semantic dependency parsing and sentiment analysis.
Contribution 1:

The question of how to combine gradient-based learning with hard decisions such as argmax is an important one for NLP. Here the question is framed within a pipeline scenario, where the training is done end-to-end, and the hard decision is one made by a parser, for example, as part of the pipeline.

Contribution 2:

Contribution 3:

Strengths

Strength argument 1:
The question is important, as argued above, and the theoretical solution (as far as I can tell) is well done.

Strength argument 2:

Strength argument 3:

Strength argument 4:

The paper is well-written, with a clear exposition of the theoretical aspects, which a number of people in the ACL community can learn from.

Strength argument 5:

The empirical results are decent, with sensible baselines and comparisons.

NLP Tasks / Applications:	N/A
Methods / Algorithms:	Strong contribution
Theoretical / Algorithmic Results:	Moderate contribution
Empirical Results:	Moderate contribution
Data / Resources:	N/A
Software / Systems:	N/A
Evaluation Methods / Metrics:	N/A
Other Contributions:	N/A
Originality (1-5):	4
Soundness/Correctness (1-5):	4
Substance (1-5):	4
Replicability (1-5):	4
Meaningful Comparison (1-5):	5
Readability (1-5):	4
Overall Score (1-6):	5
Additional Comments (Optional)

Everyone likes an acronym, of course, but where's the 'o'? Shouldn't it be SPIGET, SPIGAT, or SPIGIT?
The abstract suggests that RL requires marginal inference. Is that true?

In the discussion of RL in the intro, argument (i) - "quite expensive" - doesn't say a lot and in particular doesn't add anything to argument (ii).

Not sure I'm convinved by argument (iii) either: why can't the solution with marginalization provide an analysis by finding the MAP solution (eg most probable parse)?

Odd to describe the set {0,1} as a 'range'

I enjoyed the technical description of SPIGOT and got a lot out of sec. 2.2. The only part I failed to understand is the line which says "the projected gradients are computed using the straight-through..." - how does that relate to 4c? I'm sure I'm missing something obvious here, but the description stops at 4b.

Why does SPIGOT not assume the argmax is solved exactly? Do you just mean that this could be a heuristic beam search, for example? Please add a line to clarify.

Can you say what the PSD dataset is.


Review #2
Appropriateness:	Appropriate
Adhere to ACL 2018 Guidelines:	Yes
Adhere to ACL Author Guidelines:	Yes
Handling of Data / Resources:	Yes
Handling of Human Participants:	N/A
Summary and Contributions

Summary: The paper proposes a method for joint learning in the case of a pipeline architecture where the first stage is an argmax over a structured output space. Specifically, they propose a solution to backpropagating through the argmax which takes into consideration the constraints of the structured output space. They first compute an unconstrained update to the output of the argmax, then project this back into (a linear interpolation of) points allowed by the constraints. The resulting update to the output of the argmax is then used as the gradient to be backpropagated. Empirical evaluation on two tasks which use a parser for preprocessing show that results can be improved with this joint learning.
Contribution 1: New method for backpropagating through a structured argmax.

Contribution 2: Demonstration of improvements with joint learning when enforcing the constraints of the intermediate task.

Contribution 3: Clear and informative review of related techniques and literature.

Strengths

Strength argument 1: The paper is very clearly written, covering some very technical material at an appropriately accessible level.
Strength argument 2: The problem they address is important for NLP, given the recent trends towards joint learning of complex NLP systems.

Strength argument 3: Their solution covers an important aspect of the problem, namely how to take into consideration structured constraints in an effective method for backpropagating through argmax.

Strength argument 4: Empirical results support their claims.

Weaknesses

Weakness argument 1: The main contribution of the paper is of fairly specialised interest. The number of people in the ACL community who are interested in this issue is probably not very large.
Weakness argument 2: There is no real contribution to the big picture of what is going on when we backprop through structured argmax. This is a technical contribution situated within the existing more-or-less hacky approaches to the problem.

Weakness argument 3: One can always run more experiments.

NLP Tasks / Applications:	N/A
Methods / Algorithms:	Moderate contribution
Theoretical / Algorithmic Results:	Strong contribution
Empirical Results:	Moderate contribution
Data / Resources:	N/A
Software / Systems:	N/A
Evaluation Methods / Metrics:	N/A
Other Contributions:	N/A
Originality (1-5):	4
Soundness/Correctness (1-5):	5
Substance (1-5):	4
Replicability (1-5):	4
Meaningful Comparison (1-5):	5
Readability (1-5):	5
Overall Score (1-6):	5

Review #3
Appropriateness:	Appropriate
Adhere to ACL 2018 Guidelines:	Yes
Adhere to ACL Author Guidelines:	Yes
Handling of Data / Resources:	N/A
Handling of Human Participants:	N/A
Summary and Contributions

Summary: This paper describes a simple way to do backpropagation on functions involving an argmax over a discrete space of structures. It is similar to straight-through estimation but adds a projection step. In two tasks, this method performs generally better than STE as well as structured attention.
Contribution 1: The SPIGOT method

Contribution 2: New state of the art on semantic dependency parsing

Contribution 3:

Strengths

Strength argument 1: The proposed method is simple and should work in a wide variety of situations important in NLP.
Strength argument 2: Results are good on both tasks: syntactic plus semantic parsing, and semantic parsing plus sentiment classification.

Strength argument 3: Overall, this represents a substantial amount of solid work.

Strength argument 4:

Strength argument 5:

Weaknesses

Weakness argument 1: The justification for SPIGOT is somewhat thin. There's some intuition but not much theory. It's not a must, but whatever else the authors could provide here would be helpful.
Weakness argument 2: The acronym SPIGOT has two superfluous letters.

Weakness argument 3:

Weakness argument 4:

Weakness argument 5:

Questions to Authors (Optional)

Question 1: The idea behind SPIGOT makes some intuitive sense, but can more be said to justify it? For example, is the proxy gradient the gradient of some smooth approximation of L, or something like that?
Question 2: In equation 4a, must \eta be the same as the learning rate used in SGD on L, or is it independent? If independent, how do you choose \eta?

Question 3: To me, equation 4c is reminiscent of the perceptron update. Is there anything to that analogy?

NLP Tasks / Applications:	Strong contribution
Methods / Algorithms:	Strong contribution
Theoretical / Algorithmic Results:	Moderate contribution
Empirical Results:	Strong contribution
Data / Resources:	N/A
Software / Systems:	Strong contribution
Evaluation Methods / Metrics:	N/A
Other Contributions:	N/A
Originality (1-5):	4
Soundness/Correctness (1-5):	4
Substance (1-5):	5
Replicability (1-5):	4
Meaningful Comparison (1-5):	5
Readability (1-5):	5
Overall Score (1-6):	5


